Fine-tuning Reinforcement Learning Models is Secretly a Forgetting Mitigation Problem

Fine-tuning is a widespread technique that allows practitioners to transfer pre-trained capabilities, as recently showcased by the successful applications of foundation models. However, fine-tuning reinforcement learning (RL) models remains a challenge. This work conceptualizes one specific cause of poor transfer, accentuated in the RL setting by the interplay between actions and observations: forgetting of pre-trained capabilities. Namely, a model deteriorates on the state subspace of the downstream task not visited in the initial phase of fine-tuning, on which the model behaved well due to pre-training. This way, we lose the anticipated transfer benefits. We identify conditions when this problem occurs, showing that it is common and, in many cases, catastrophic. Through a detailed empirical analysis of the challenging NetHack and Montezuma's Revenge environments, we show that standard knowledge retention techniques mitigate the problem and thus allow us to take full advantage of the pre-trained capabilities. In particular, in NetHack, we achieve a new state-of-the-art for neural models, improving the previous best score from $5$K to over $10$K points in the Human Monk scenario.

==> nethack_small_model_exps.tex <==

\section{NetHack analysis on a smaller model}
\label{app:nethack_results}

\subsection{Setup}
\paragraph{Dataset} This paper uses a subset of the NetHack Learning Dataset (NLD) collected by~\cite{hambrodungeons} called NLD-AA. It contains over 3 billion state-action-score trajectories and metadata from 100,000 games collected from the winning bot of the NetHack Challenge~\cite{hambro2022insights}.
% \bartek{ we use this dataset, but we only train on human monk (makes about 8k games)} 
In particular, we use about 8000 games of Human Monk. This character was chosen because it was extensively evaluated in the previous work \cite{hambrodungeons} and because the game setup for the Human Monk is relatively straightforward, as it does not require the agent to manage the inventory. 
% \maciek{1705: It would be nice to have one sentence explaining why we are using Human Monk, either here or in the next paragraph (it's the easiest setup and that's what prior work did).} 
The bot is based on the 'AutoAscend' team solution, a symbolic agent that leverages human knowledge and hand-crafted heuristics to progress in the game. Its decision-making module is based on a behavior tree model.

% Models used and architecture
\paragraph{Architecture} % For the online training in NLE
% \maciek{1705: maybe specify that you mean online NLE here, not the dataset learning},
We use the solution proposed by the 'Chaotic Dwarven GPT-5' team, which is based on Sample Factory~\cite{Petrenko2020SampleFE} that was also used in~\cite{hambrodungeons}. 
This model utilizes an LSTM architecture that incorporates representations from three encoders, which take observations as inputs. The LSTM network's output is then fed into two separate heads: a policy head and a baseline head. The model architecture used both in online and offline settings consists of a joint backbone for both actor and critic. It takes as an input three components: RGB image of the main game screen, \verb|blstats|, and \verb|message|. Where \verb|blstats| refers to the player's status information, such as health and hunger, and \verb|message| refers to the textual information displayed to the player, such as notifications and warnings. These inputs are processed separately using the Nature DQN CNN~\cite{mnihHumanlevelControlDeep2015} for the image input and fully connected layers for the \verb|blstats| and \verb|message| inputs and are merged before passing to LSTM. This baseline allows for fast training
% \maciek{1805: faster than what? I don't quite get that}
but struggles with learning complex behaviours required for certain roles in the game. Thus, we choose only high-performing Human Monk character. More details about the architecture can be found in~\cite{Petrenko2020SampleFE}. The model hyperparameters are shown in Table~\ref{tab:hparams_nle} -- analogical to Table 6 from~\cite{Petrenko2020SampleFE}. 


%Methods
\paragraph{Pre-training}
During the offline pre-training phase, we employed Behavioral Cloning (BC)~\cite{bain1995framework,ross2010efficient}, an imitation learning approach that utilizes a supervised learning objective to train the policy to mimic the actions present in the dataset. To be more specific, it utilizes cross entropy loss function between the policy action distribution and the actions from the NLD-AA dataset. The offline procedure was conducted with the hyperparameters from Table~\ref{tab:hparams_nle}, except: \verb|actor_batch_size=256|, \verb|batch_size=128|, \verb|ttyrec_batch_size=512| and \verb|adam_learning_rate=0.001| for two billions steps. For more details on hyperparameters, please refer to the original article~\cite{Petrenko2020SampleFE}.

\subsection{Results}

\piotrm{28.01 I assume this will be review subject to the new expeirmental section.}

In this section, we provide additional results for the NetHack experiments.

\diff{\paragraph{Different approaches to distillation} In our main NetHack experiments, we use the following behavioral cloning loss:
\begin{equation}
    \mathcal L_{BC}(\theta) = \mathbb{E}_{s \sim \mathcal{B}} [ D_{KL}^s\infdivx{\pi_*(\cdot \vert s)}{\pi_\theta(\cdot \vert s)} ],
\end{equation}
where $\mathcal{B}$ is a buffer of data gathered by the AutoAscend, and $\pi_*$ is the pre-trained policy. However, there are more possible ways to apply distillation to this problem. Here, we study two other approaches -- \textbf{Kickstarting} and \textbf{Behavioral Cloning with Expert Labels}. 
}

\diff{In \textbf{Kickstarting} (KS)~\cite{schmitt2018kickstarting}, we use a very similar loss, but now we apply KL on the data gathered online by the student. More formally:
\begin{equation}
    \mathcal L_{KS}(\theta) = \mathbb{E}_{s \sim \mathcal{B}_\theta} [ D_{KL}^s\infdivx{\pi_*(\cdot \vert s)}{\pi_\theta(\cdot \vert s)} ],
\end{equation}
where $\mathcal{B}_\theta$ denotes a buffer of data gathered by the online policy $\pi_\theta$.}

In \textbf{Behavioral Cloning with Expert Label} (BCEL), we use the states gathered by the expert, same as in behavioral cloning, but we use a different target. Namely, we use the prediction from the AutoAscend dataset on which we pre-trained $\pi^*$. Formally,
\begin{equation}
    \mathcal L_{BCEL}(\theta) = \mathbb{E}_{s \sim \mathcal{B}} [ D_{KL}^s\infdivx{y^*}{\pi_\theta(\cdot \vert s)}],
\end{equation}
where $y^*$ is the label from the AutoAscend dataset corresponding to the action taken by the expert agent. As such, there is a subtle difference between $\mathcal L_{BC}$ and $\mathcal L_{BCEL}$. In the first one, we attempt to preserve the knowledge of $\pi^*$, in the second one we try to optimize the same loss that was used to train $\pi^*$. If $\pi^*$ were to perfectly clone the AutoAscend dataset, these two approaches would be exactly the same, but in practice, we see that there is a significant discrepancy between these two. The $\mathcal L_{BCEL}$ formulation also corresponds to the BCO approach from \cite{hambrodungeons}, although in that work the authors did not consider the transfer of parameters at all. To differentiate between these approaches in the following text, we call fine-tuning with the $\mathcal L_{BC}, \mathcal L_{KS}$, and $\mathcal L_{BCEL}$ losses respectively APPO-BC, APPO-KS and APPO-BCEL. APPO-FT is vanilla-finetuning, and APPO is training from scratch. 


We compare these approaches and show the results in Figure~\ref{fig:nethack_full_train_appendix} and Figure~\ref{fig:nethack_per_level_appendix}. First of all, we observe that APPO-KS performs worse than the other types of distillation. We attribute this gap to the fact that APPO-KS applies regularization on the online data not seen during the pre-training, where the pre-trained policy performs poorly. The regularization stops the model from learning a better behavior on these states and as such leads to stagnation. On the other hand, quite surprisingly, APPO-BCEL performs slightly worse than APPO-BC, even though it uses targets from the AutoAscend dataset that performs much better than $\pi^*$. We hypothesize that it is simpler for the model to maintain the initial performance with APPO-BC rather than to learn something new with APPO-BCEL. 


\begin{figure}
    \centering
    \mute{\includegraphics[width=0.7\textwidth]{imgs/nethack_new/nethack_full_train_appendix.png}}
    \caption{\diff{\small Average return when fine-tuning on NetHack with additional distillation approaches.}
    }
    \label{fig:nethack_full_train_appendix}
\end{figure}

\begin{figure}
    \centering
    \mute{\includegraphics[width=\textwidth]{imgs/nethack_new/nethack_levels_v4_appendix.png}}
    \caption{\diff{\small Average return of each of each NetHack method throughout the training with additional approaches to distillation, evaluated when started on a specific dungeon level. The top row shows the initial phase of the training (up to 100M steps), and the bottom row shows the full training (up to 2B steps, note the x-axis scale change).  While the distillation approaches showed similar performance in the early stages (top row), APPO-BC stands out in the overall training, particularly on Level 2 and Level 4.}
    }
    \label{fig:nethack_per_level_appendix}
\end{figure}

These results show that one should carefully choose how to apply distillation to the model. At the same time, we do not claim that these rankings will transfer to other settings and that APPO-BC is inherently better than APPO-BCEL and APPO-KS. We believe that one could fix APPO-KS by e.g. decaying the regularization term as the training goes on.



\paragraph{Forgetting in the fine-tuned models} In Figure~\ref{fig:log_forgetting_nethack}, we measure how different methods forget throughout the fine-tuning process. In particular, we measure the KL divergence on the data generated by the teacher (the pre-trained model). While APPO-FT forgets completely, APPO-BC keeps the divergence at fairly low levels. 




% \paragraph{Enabling forgetting in APPO-KS} In the main part of this paper, we showed that APPO-KS underperforms on the fine-tuning task (see Figure~\ref{fig:nethack_results}). Here, we show that the results can be substantially improved by limiting knowledge retention (i.e., allowing for forgetting). In particular, we introduce a decay term that reduces the weight of the KS term by multiplying it by $\gamma^t$, where $\gamma$ is the decay hyperparameter and $t$ is the number of gradient steps. Results presented in Figure~\ref{fig:nethack_ks_decay} show that one can regain good performance by reducing the regularization strength as time goes by. This result highlights that knowledge retention methods should be applied cautiously. 

\paragraph{Descent statistics} Although the obtained return is a valuable metric of the performance of a policy, it is far from the only one. Here, for each of the policies introduced in our experiments, we check the performance in terms of the number of levels visited by each policy. The results are shown in Figure~\ref{fig:nethack_levels}.

\begin{figure}
    \centering
    \mute{\includegraphics[width=0.6\textwidth]{imgs/appendix/nethack_sokoban_freq.png}}
    \caption{\diff{The distribution of how many pits the agent manages to fill in the Sokoban levels.}}
    \label{fig:sokoban_freq}
\end{figure}

\paragraph{Sokoban results and discussion}  Here, we discuss the Sokoban levels in NetHack and their unique complexity. In the Sokoboan levels, the player has to face monsters and essentially play the game as normal in addition to moving boulders. There are specific unlucky scenarios when the monster will spawn between boulder and pit, which require the agent to find non-trivial ways of killing the monster from behind the boulder. Additionally, the Sokoban levels are encountered fairly late in the game and as such might be relatively underrepresented in the data.

\diff{As such, the pre-trained agent that clones the actions of an expert policy starts with a score of 1.5 filled pits. It is worth noting that the mean is somewhat skewed due to the number of episodes when the agent chooses to ignore Sokoban completely and go into a different branch of the dungeon. This is a viable strategy, since the agent might try to increase the score in a different manner. In Figure~\ref{fig:sokoban_freq}, we show a histogram of the number of pits filled by the pre-trained agent. It is worth highlighting that it does not progress at the problem in over $50\%$ of trajectories, but in over $25\%$ percent of trajectories it solves at least half of the level.}

\begin{figure}
    \centering
    \mute{\includegraphics[width=0.6\textwidth]{imgs/appendix/nethack_long_appo.png}}
    \caption{Training from scratch on NetHack, ran with twice the budget of other methods. Although it manages to outperform APPO-FT, APPO-BC still achieves a better results, even with the smaller timestep budget.}
    \label{fig:appo_4b}
\end{figure}

\newdiff{\paragraph{Training from scratch with more steps} Although in our experiments we observe that fine-tuning with knowledge distillation methods significantly outperforms training from scratch with a given budget of timesteps, it is not clear if a model trained from scratch can finally catch up given enough timesteps. To investigate this, we run APPO with $4$B steps rather than $2$B as in the previous experiments. In Figure~\ref{fig:appo_4b}, we compare it with pure fine-tuning. We observe that although APPO manages to finally overtake pure fine-tuning, in the end it still falls short of knowledge retention-based APPO-BC that achieved score of over 3500. }

% The analysis of the number of levels visited by each policy in Figure~\ref{fig:nethack_levels} reveals an interesting pattern. Despite APPO-KS underperforming in terms of episode return, it explores the dungeon to greater depths, resulting in higher returns in later stages. However, its weaker performance on initial levels decreases its average performance. This highlights the challenge of effectively leveraging valuable knowledge from a pretrained model, as it is difficult to determine what should be retained.

\paragraph{Full results} In Figure~\ref{fig:nethack_full_results} we show the full results of our fine-tuning experiments with evaluation on specific levels. In addition to the standard average return metrics, we provide additional information such as the score wrt. to other objectives defined in NLE~\cite{kuttler2020nethack} (e.g. eating food, gathering gold, descending through the dungeon) and additional player statistics (experience level, energy).

% \paragraph{EWC performance} For brevity, we did not discuss the performance of APPO-EWC in the main text. Here, in Figure~\ref{fig:nethack_ewc} we show that APPO-EWC achieves similar results as APPO-FT, i.e. vanilla fine-tuning.



\begin{figure}[H]
    \centering
    \mute{\mute{\includegraphics[width=0.8\textwidth]{imgs/appendix/nethack_kl_div_v2.png}}}

    \caption{ We measure how outputs of the policy change to the pre-trained one during training every 100 million steps, note the log-scale. We can see that APPO-BC aggressively prevents changes to the policy. 
    % On the other hand, regularization-based EWC permits significant changes since it makes a relatively small contribution to the loss function due to the scaling factor. % \michalb{TODO: Add EWC}
    } 
    \label{fig:log_forgetting_nethack}
\end{figure}

% \begin{figure}[H]
%     \centering
%     \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_ks_decay.png}}
%     \caption{(Left) Average success rate for APPO-KS with different decay strategies. (Right) The regularization coefficient's value depends on the timestep for different $\gamma$ values.}
%     \label{fig:nethack_ks_decay}
% \end{figure}

\begin{figure}[H]

    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_bc_v2.png}}
        \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_v2.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_ft_v2.png}}
        \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_bc_v2.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_ewc_v2.png}}
        \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_ks_v2.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_bcel_v2.png}}
    \end{subfigure}
    % \begin{subfigure}[b]{\textwidth}
    %     \centering
    %     % \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_ks_t.png}}
    %     % \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_bc_t.png}}
    %     % \mute{\includegraphics[width=.44\columnwidth]{imgs/appendix/levels_reached_appo_ewc_t.png}}
    % \end{subfigure}
\caption{Average percentage of levels reached by different methods. The red line shows the average return obtained in trajectories that finished on this level, while the blue bar shows the percentage of trajectories that reached a given level.}
\label{fig:nethack_levels}

\end{figure}%



\begin{figure}[H]
\caption{NetHack performance on various metrics when starting from specific levels}
\label{fig:nethack_full_results}

    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/None.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/saves2.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/saves3.png}}
    \end{subfigure}
    
\end{figure}%
\begin{figure}[H]\ContinuedFloat
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/saves4.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/saves5.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/saves6.png}}
    \end{subfigure}
\end{figure}%
\begin{figure}[H]\ContinuedFloat

    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/saves7.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/saves8.png}}
    \end{subfigure}
    \begin{subfigure}[b]{\textwidth}
        \centering
        \mute{\includegraphics[width=\textwidth]{imgs/appendix/nethack_levels/saves9.png}}
    \end{subfigure}
\end{figure}


